Universally Composable Quantum Multi-Party Computation

The Universal Composability model (UC) by Canetti (FOCS 2001) allows for secure composition of arbitrary protocols. We present a quantum version of the UC model which enjoys the same compositionality guarantees. We prove that in this model statistically secure oblivious transfer protocols can be constructed from commitments. Furthermore, we show that every statistically classically UC secure protocol is also statistically quantum UC secure. Such implications are not known for other quantum security definitions. As a corollary, we get that quantum UC secure protocols for general multi-party computation can be constructed from commitments.

==> macros.tex <==
\newcommand\includeonlyonceYTEROGFJSDFVJNICXERPRYDEKFC{}

\makeatletter

\newcommand\Hilbert[1]{\calH^\mathit{#1}}
\newcommand\Hbits{\Hilbert{bits}}
\newcommand\Hstate{\Hilbert{state}}
%\newcommand\Haddr{\Hilbert{addr}}
%\newcommand\Hcomm{\Hilbert{comm}}
\newcommand\Hclass{\Hilbert{class}}
\newcommand\Hquant{\Hilbert{quant}}
%\newcommand\Hsender{\Hilbert{sender}}
%\newcommand\Hrcpt{\Hilbert{rcpt}}
%\newcommand\Hfrom{\Hilbert{from}}
%\newcommand\Hto{\Hilbert{to}}
\newcommand\calH{\mathcal H}
\newcommand\calP{\mathcal P}
\newcommand\setC{\mathbbm C}
\newcommand\bits[1]{\bit^{#1}}
\newcommand\bit{\{0,1\}}
\newcommand\calE{\mathcal E}
\newcommand\calC{\mathcal C}
\newcommand\calO{\mathcal O}
\newcommand\id{\mathit{id}}
\newcommand\calZ{\mathcal Z}
\newcommand\bfN{\mathbf N}
\newcommand\setN{\mathbbm N}
\newcommand\ids{\mathit{ids}}
%\newcommand\calD{\mathcal D}
\newcommand\Exec{\mathrm{Exec}}
%\newcommand\calA{\mathcal A}
%\newcommand\calS{\mathcal S}
\newcommand\babs[1]{\bigl\lvert#1\bigr\rvert}
\newcommand\abs[1]{\lvert#1\rvert}
\newcommand\base{\{+,\times\}}
\newcommand\bases[1]{\base^{#1}}
\newcommand\ket[1]{\lvert #1\rangle}
\newcommand\bra[1]{\langle #1\rvert}
\newcommand\butter[1]{\ket{#1}\bra{#1}}
\newcommand\braket[2]{\langle#1\vert#2\rangle}
\newcommand\calF{\mathcal F}
\newcommand\calG{\mathcal G}
\newcommand\FCOM{\calF_\mathrm{COM}}
\newcommand\FOT{\calF_\mathrm{OT}}
\newcommand\FROT{\calF_\mathrm{ROT}}
\newcommand\FSMT{\calF_\mathrm{SMT}}
\newcommand\FAND{\calF_\mathrm{AND}}
\newcommand\parties{\mathit{parties}}
\newcommand\piQOT{\pi_\mathrm{QOT}}
\newcommand\piQROT{\pi_\mathrm{QROT}}
\newcommand\Adv{\mathrm{Adv}}
\newcommand\Advd{\Adv_\mathit{dummy}}
\newcommand\Advdc{\Advd^\mathit{class}}
\newcommand\Sim{\mathrm{Sim}}
\newcounter{step}
\newcommand\nextstep[1]{\medskip\noindent
  \refstepcounter{step}\label{#1}%
  \textbf{Game~\arabic{step}.}}
\newcommand\stepautorefname{Game}
\newcommand\FFC{\calF_\mathrm{FakeCOM}}
\let\TIlde\Tilde
\newcommand\com{\mathrm{com}}
\DeclareMathOperator\tr{tr}
\newcommand\Eclass{\calE_\mathit{class}}
\newcommand\Einit{\calE_\mathit{init}}
\newcommand\idrcpt{\id_\mathit{rcpt}}
\newcommand\idsender{\id_\mathit{sender}}
\newcommand\environment{\mathtt{environment}}
\newcommand\adversary{\mathtt{adversary}}
\newcommand\rmOne{\rmNum{I}}
\newcommand\rmTwo{\rmNum{II}}
\newcommand\rmThree{\rmNum{III}}
\newcommand\rmFour{\rmNum{IV}}
\newcommand\rmFive{\rmNum{V}}
\newcommand\rmSix{\rmNum{VI}}
\newcommand\rmNum[1]{{\textrm{\textsmaller{#1}}}}
\newcommand\pagelabel[1]{\phantomsection\label{#1}}
\ifx\autopageref\undefined\newcommand\autopageref[1]{page~\ref{#1}}\fi
\newcommand\marginparx[1]{\ifinner\marginnote{#1}\else\ifx\@captype\undefined\marginpar{#1}\else\marginnote{#1}\fi\fi}
\newcommand\dotparagraph[1]{\paragraph{#1.}}
\renewcommand\subparagraph[1]{\medskip\noindent\textit{#1}}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "quantum-uc-ot"
%%% End: 

